Teacher-Student Learning based Low Complexity Relay Selection in Wireless Powered Communications

Radio Frequency Energy Harvesting (RF-EH) networks are key enablers of massive Internet-of-things by providing controllable and long-distance energy transfer to energy-limited devices. Relays, helping either energy or information transfer, have been demonstrated to significantly improve the performance of these networks. This paper studies the joint relay selection, scheduling, and power control problem in multiple-source-multiple-relay RF-EH networks under nonlinear EH conditions. We first obtain the optimal solution to the scheduling and power control problem for the given relay selection. Then, the relay selection problem is formulated as a classification problem, for which two convolutional neural network (CNN) based architectures are proposed. While the first architecture employs conventional 2D convolution blocks and benefits from skip connections between layers; the second architecture replaces them with inception blocks, to decrease trainable parameter size without sacrificing accuracy for memory-constrained applications. To decrease the runtime complexity further, teacher-student learning is employed such that the teacher network is larger, and the student is a smaller size CNN-based architecture distilling the teacher's knowledge. A novel dichotomous search-based algorithm is employed to determine the best architecture for the student network. Our simulation results demonstrate that the proposed solutions provide lower complexity than the state-of-art iterative approaches without compromising optimality.

==> tex_files/optimality.tex <==

\subsection{Optimality Conditions}

This section analyzes the optimality conditions of the problem. The resulting conditions will later be used to design deep learning architectures.

\begin{lemma}  \label{lemma:dec} Let $\{\hat{\tau}_0^i, \hat{\tau}_{S_i}^{AP}\}$  be the solution pair of the single source problem corresponding to $S_i$ for direct transmission to AP  for $i = 1,\ldots,N$. $\hat{\tau}_0^i$ and $\hat{\tau}_{S_i}^{AP}$ are decreasing functions of $ \phi_{S_i}^{AP} = \frac{g_{S_i}^{AP}  (\Psi_{S_i} - M_{S_i}\Omega_{S_i})}{({1-\Omega_{S_i}})}$ \label{lemma:EHandGamma}. 
\end{lemma}

\begin{proof}
The solution pair $\{\hat{\tau}_0^i, \hat{\tau}_{S_i}^{AP}\}$ is expressed by  
\begin{align} 
&\hat{\tau}_0^i =  \frac{D\ln(2)}{W\alpha_{S_1}}, \label{eq:ITwoR} \\
& \hat{\tau}_{S_i}^{AP}=\frac{\tau_{S_1}}{\gamma_{S_1}}(2^{\frac{D_{S_1}}{W\tau_{S_1}}}-1)\label{eq:EHwoR} 
\end{align}
where 
$ \gamma_{S_i} = \frac{g_{S_1}  (\Psi_{S_i} - M_{S_i}\Omega_{S_i})}{({1-\Omega_{S_i}})WN_0}$, $ \alpha_{S_i} = \mathbb{L}_0 \left(\frac{\gamma_{S_1}-1}{e}\right) +1$, and $\mathbb{L}_0(.) $ is the Lambert W-function in 0 branch \cite{Onalan2020}.  Note that $\gamma_{S_i}$ is propotional to $\phi_{S_i}^{AP}$.  The first derivative of Eq.~(\ref{eq:ITwoR}) and (\ref{eq:EHwoR}) with respect to $\gamma_{S_i}$ are negative \cite{Onalan2020}. Then, Eqs.~(\ref{eq:ITwoR}) and (\ref{eq:EHwoR}) decreasing functions of $\gamma_{S_i}$ so $\phi_{S_i}^{AP}$.  

\end{proof}

\begin{claim} \label{lemma:relCond} Under the moderate and high AWGN, the necessary condition for relay selection $R_1$ at source $S_1$ is 
\begin{equation}
	\min \left(g_{S_1}^{R_1}\phi_{S_1}^{AP}, g_{R_1}^{AP}\phi_{S_1}^{AP} \right) > g_{S_1}^{AP}\phi_{S_1}^{AP}.
	\label{eq:relSelCondGeneral} 
\end{equation}
\end{claim}





\begin{claim}
In single-source-multiple-relay networks, the relay selection criterion of $S_i$ can be defined as 
\begin{equation}
\argmax_j \min \left(g_{S_i}^{R_j}\phi_{S_i}^{AP}, g_{R_j}^{AP}\phi_{R_j}^{AP} \right)
\label{eq:relaySelectCriteria}
\end{equation}
\end{claim}

Note that Eq.~(\ref{eq:relaySelectCriteria}) is in parallel to the commonly adapted opportunistic relaying (OR) criterion, which  jointly considers the channel conditions of source-to-relay and relay-to-AP links \cite{Bletsas2006}. 

==> tex_files/param_table.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|cccc|cccc|cccc|}
\hline
  &   &             & \multicolumn{4}{c|}{SC-NET}                                                                                                                                                                   & \multicolumn{4}{c|}{MINI-SC\_NET and   STU-SC-NET}                                                                                                                                            & \multicolumn{4}{c|}{SKIN-NET}                                                                                                                                                                             \\ \hline
N & K & input\_size & \multicolumn{1}{c|}{L\_C} & \multicolumn{1}{c|}{Number of nodes per layer} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}kernel \\      (c\_1 x c\_2)\end{tabular}} & Trainable parameters & \multicolumn{1}{c|}{L\_C} & \multicolumn{1}{c|}{Number of nodes per layer} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}kernel \\      (c\_1 x c\_2)\end{tabular}} & Trainable parameters & \multicolumn{1}{c|}{L\_I} & \multicolumn{1}{c|}{Number of nodes per layer} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}kernel \\      (k\_1 x k\_2),(k\_3xk\_4)\end{tabular}} & Trainable parameters \\ \hline
1 & 2 & 2x4         & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{16,64,64,32,32,16,10}      & \multicolumn{1}{c|}{2x2}                                                                  & 36,457               & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{2,2,10}                    & \multicolumn{1}{c|}{2x2}                                                                  & 145                  & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{32,64,64,32,24,16}         & \multicolumn{1}{c|}{4x4,2x2}                                                                          & 24,261               \\ \hline
2 & 2 & 3x4         & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{16,64,64,32,32,16,10}      & \multicolumn{1}{c|}{3x2}                                                                  & 55,131               & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{2,2,10}                    & \multicolumn{1}{c|}{2x2}                                                                  & 277                  & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{32,64,64,32,24,16}         & \multicolumn{1}{c|}{4x4,3x2}                                                                          & 25,517               \\ \hline
3 & 2 & 4x4         & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{16,64,64,32,32,16,10}      & \multicolumn{1}{c|}{3x3}                                                                  & 86,391               & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{2,2,10}                    & \multicolumn{1}{c|}{2x2}                                                                  & 808                  & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{32,64,64,32,24,16}         & \multicolumn{1}{c|}{4x4,3x3}                                                                          & 27,401               \\ \hline
4 & 2 & 5x4         & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{16,64,64,32,32,16,10}      & \multicolumn{1}{c|}{4x4}                                                                  & 166,543              & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{2,2,10}                    & \multicolumn{1}{c|}{2x2}                                                                  & 2,779                & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{32,64,64,32,24,16}         & \multicolumn{1}{c|}{4x4,4x4}                                                                          & 31,797               \\ \hline
5 & 2 & 6x4         & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{16,64,64,32,32,16,10}      & \multicolumn{1}{c|}{5x4}                                                                  & 272,945              & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{2,2,10}                    & \multicolumn{1}{c|}{2x2}                                                                  & 10,069               & \multicolumn{1}{c|}{5}    & \multicolumn{1}{c|}{32,64,64,32,24,16}         & \multicolumn{1}{c|}{4x4,5x5}                                                                          & 37,449               \\ \hline
\end{tabular}
\end{table}

==> tex_files/relaxed_prob.tex <==
\subsection{Relaxed Problem}

The relaxation of Problem~(\ref{eq:relSel}) is obtained as follows.  The integrality constraint  Eq.~(\ref{eq:relSel:integrality}) of Problem~(\ref{eq:relSel}) is relaxed as $0 \leq b_i^j \leq 1$. This relaxation allows $b_i^j$ to take fractional values for $i=1,\ldots,N$ and $j=0,\ldots,K$.

In Problem~(\ref{eq:relSel}), $P_{S_i}^{R_j} \tau_{S_i}^{R_j}$ and $P_{R_j}^{AP} \tau_{R_j}^{AP}$ are replaced by new variables $A_{S_i}^{R_j}$ and $A_{R_j}^{AP}$, respectively, so that constraints (\ref{eq:relSel:energy1})-(\ref{eq:relSel:demand2}) represent convex sets. 


After the replacement,  Eqs.~(\ref{eq:relSel:maxpow1}) and (\ref{eq:relSel:maxpow2}) include a product of two variables (e.g., $b_i^j \tau_{S_i}^{R_j}$ and $b_i^j \tau_{R_j}^{AP}$), which causes the non-convexity. Instead of these products, we define their convex/concave envelopes, lower and upper bounding constraints, which is a common relaxation technique proposed in \cite{PietroBelotti2012}. Now, the relaxed problem can be solved by a convex optimization tool, e.g., CVX \cite{cvx}. 

\begin{subequations} \label{eq:relSel}
\begin{align}
\min \qquad &  \tau_0 + \sum_{i=1}^N \sum_{j=0}^K \tau_{S_i}^{R_j} + \sum_{j=1}^K \tau_{R_i}^{AP} \label{eq:relax:obj} \\
\text{s.t.}\qquad & \sum_{j=0}^K b_i^j = 1, \qquad i=1,\ldots,N, \label{eq:relax:relSel}\\
									& A_{S_i}^{R_j}  \leq P^{max} b_i^j\tau_{S_i}^{R_j}, \quad i=1,\ldots,N, \; j=0,\ldots,K, \label{eq:relax:maxpow1} \\
									&  A_{R_j}^{AP} \leq  \min \left\{P^{max}\tau_{R_j}^{AP},P^{max}\tau_{R_j}^{AP} \sum_{i=1}^N  b_i^j \right\}, \nonumber \\ 
									&\hspace{4.4cm} j=0,\ldots,K, \label{eq:relax:maxpow2} \\
									& A_{S_i}^{R_j} \leq \frac{ \Psi_{S_i} - M_{S_i}\Omega_{S_i}}{1-\Omega_{S_i}}\tau_0 , \qquad i=1,\ldots,N, \nonumber \\ 
									& \hspace{4.4cm} j=0,\ldots,K, \label{eq:relax:energy1} \\
									& A_{R_j}^{AP} \leq \frac{ \Psi_{R_j} - M_{R_j}\Omega_{R_j}}{1-\Omega_{R_j}}\tau_0 , \qquad j=1,\ldots,K, \label{eq:relax:energy2}\\
									& \tau_{S_i}^{R_j} W \log_2 \left( 1 + \frac{P_{S_i}^{R_j}g_{S_i}^{R_j}}{WN_0} \right)\geq D_{S_i}b_i^j, \quad \nonumber \\ & \hspace{2.4cm} i=1,\ldots,N, \; j=0,\ldots,K,  \label{eq:relax:demand1}\\
									& \tau_{R_j}^{AP} W \log_2 \left( 1 + \frac{P_{R_j}^{AP}g_{R_j}^{AP}}{WN_0} \right) \geq \sum_{i=1}^N  D_{S_i}b_i^j, \nonumber \\ & \hspace{4.4cm} j=0,\ldots,K, \label{eq:relax:demand2}\\							
									&  \tau_0,\tau_{R_j}^{AP}, P_{R_j}^{AP},\tau_{S_i}^{R_j}, P_{S_i}^{R_j} \geq 0, \quad i=1,\ldots,N, \; \nonumber \\ & \hspace{4.6cm} j=1,\ldots,K, \label{eq:relSel:nonneg}\\
									& 0 \leq b_i^j \leq 1,  \quad i=1,\ldots,N, \; j=1,\ldots,K.		\label{eq:relax:integrality}	
\end{align}
\end{subequations}
